Think Before You Duel: Understanding Complexities of Preference Learning under Constrained Resources

We consider the problem of reward maximization in the dueling bandit setup along with constraints on resource consumption. As in the classic dueling bandits, at each round the learner has to choose a pair of items from a set of $K$ items and observe a relative feedback for the current pair. Additionally, for both items, the learner also observes a vector of resource consumptions. The objective of the learner is to maximize the cumulative reward, while ensuring that the total consumption of any resource is within the allocated budget. We show that due to the relative nature of the feedback, the problem is more difficult than its bandit counterpart and that without further assumptions the problem is not learnable from a regret minimization perspective. Thereafter, by exploiting assumptions on the available budget, we provide an EXP3 based dueling algorithm that also considers the associated consumptions and show that it achieves an $\tilde{\mathcal{O}}\left({\frac{OPT^{(b)}}{B}}K^{1/3}T^{2/3}\right)$ regret, where $OPT^{(b)}$ is the optimal value and $B$ is the available budget. Finally, we provide numerical simulations to demonstrate the efficacy of our proposed method.

==> sec/App_proof_of_regret_bound_con.tex <==
\begin{proof}

Recall that we have $\displaystyle W_{x, t}(k) = \exp\left(\eta\sum_{s=1}^{t - 1} \hat{\ell}_{x,s}(k)\right)$. Therefore,
\begin{align*}
    \sum_{k = 1}^K W_{x,t + 1}(k)
    &= \sum_{k = 1}^K W_{x,t}(k) \exp(\eta \hat{\ell}_{x,t}(k)) \\
    &= \Big(\sum_{j=1}^{K}W_{x,t}(j)\Big) \sum_{k=1}^K \frac{W_{x, t}(k)}{\sum_{j=1}^{K}W_{x,t}(j)} \exp\big(\eta \hat{\ell}_{x, t}(k)\big) \\
   &= W \sum_{k=1}^K \frac{W_{x, t}(k)}{W} \exp\big(\eta \hat{\ell}_{x, t}(k)\big)\\
   &= W \sum_{k=1}^K \frac{p_{x,t}(k) - \frac{\gamma}{K}}{1-\gamma} \exp\Bigg(\underbrace{\eta \bigg[\hat{s}_t(i) + Z \lambda_{t}^{\top} \Big(\frac{B}{T}\mathbbm{1} - \hat{u}_t(i) \Big)\bigg]}_{I}\Bigg)
\end{align*}
where $W = \sum_{j=1}^{K}W_{x,t}(j)$. Now consider term $I$.
\begin{align*}
    \eta \bigg[\hat{s}_t(i) + Z \lambda_{t}^{\top} \Big(\frac{B}{T}\mathbbm{1} - \hat{u}_t(i) \Big)\bigg] \leq \eta
\end{align*}
\begin{align*}
     a \leq &\overset{(a)}{=} W_{+1, t} \sum_{k=1}^K \frac{p_{+1, t}(k) - \gamma/K}{1 - \gamma} \exp(\eta \hat{g}_{+1, t}(k)) \\
    &\overset{(b)}{\leq} W_{+1, t} \sum_{k=1}^K \frac{p_{+1, t}(k) - \gamma/K}{1 - \gamma} (1 + \eta \hat{g}_{+1, t}(k) + \eta^2 \hat{g}^2_{+1, t}(k)) \\
    &\leq W_{+1, t} \left(1 + \frac{\eta}{1 - \gamma} \sum_{k=1}^K p_{+1, t}(k) \hat{g}_{+1, t}(k) + \frac{\eta^2}{1 - \gamma} \sum_{k=1}^K p_{+1, t}(k) \hat{g}^2_{+1, t}(k) \right) \\
    &\overset{(c)}{\leq} W_{+1, t} \exp\left(\frac{\eta}{1 - \gamma} \sum_{k=1}^K p_{+1, t}(k) \hat{g}_{+1, t}(k) + \frac{\eta^2}{1 - \gamma} \sum_{k=1}^K p_{+1, t}(k) \hat{g}^2_{+1, t}(k) \right)
\end{align*}
Here, $(a)$ follows from the definition of $p_{+1, t}(k)$ in Algorithm \ref{alg:3p}. Note that, by assumption on $\eta$, $\beta$, $\gamma$, and $K$
\begin{align*}
    \eta \hat{g}_{+1, t}(k) \leq \eta \frac{1 + \beta}{p_{+1, t}(k)} \leq \eta K\frac{1 + \beta}{\gamma} \leq 1.
\end{align*}
Thus, $(b)$ follows from the inequality $e^x \leq 1 + x + x^2$ if $x \leq 1$. $(c)$ follows from the inequality $1 + x \leq e^x$. We now have,
\begin{align*}
    \ln \frac{W_{+1, t + 1}}{W_{+1, t}} \leq \frac{\eta}{1 - \gamma} \sum_{k=1}^K p_{+1, t}(k) \hat{g}_{+1, t}(k) + \frac{\eta^2}{1 - \gamma} \sum_{k=1}^K p_{+1, t}(k) \hat{g}^2_{+1, t}(k).
\end{align*}
Summing over $t = 1, 2, \dots, T$, we get
\begin{equation}
    \label{eq:w_ration_upper_bound_row_player}
    \ln \frac{W_{+1, T + 1}}{W_{+1, 1}} \leq \frac{\eta}{1 - \gamma} \sum_{t=1}^{T} \sum_{k=1}^K p_{+1, t}(k) \hat{g}_{+1, t}(k) + \frac{\eta^2}{1 - \gamma} \sum_{t=1}^{T} \sum_{k=1}^K p_{+1, t}(k) \hat{g}^2_{+1, t}(k).
\end{equation}
Note that, $W_{+1, 1} = K$ (see Algorithm \ref{alg:3p}). For any action $j \in [K]$,
\begin{equation}
    \label{eq:w_ration_lower_bound_row_player}
    \ln \frac{W_{+1, T + 1}}{W_{+1, 1}} \geq \ln W_{+1, T + 1}(j) - \ln K = \eta\sum_{t=1}^T \hat{g}_{+1, t}(j) - \ln K
\end{equation}
Combining \eqref{eq:w_ration_upper_bound_row_player} and \eqref{eq:w_ration_lower_bound_row_player} gives
\begin{equation*}
    \sum_{t=1}^T \hat{g}_{+1, t}(j) \leq \frac{1}{1 - \gamma} \sum_{t=1}^T \sum_{k=1}^K p_{+1, t}(k) \hat{g}_{+1, t}(k) + \frac{\eta}{1 - \gamma} \sum_{t=1}^T \sum_{k=1}^K p_{+1, t}(k) \hat{g}^2_{+1, t}(k) + \frac{\ln K}{\eta}.
\end{equation*}
Now consider the sum $\sum_{k=1}^K p_{+1, t}(k) \hat{g}_{+1, t}(k)$.
\begin{equation}
    \label{eq:hat_g_expectation}
    \sum_{k=1}^K p_{+1, t}(k) \hat{g}_{+1, t}(k) = \sum_{k=1}^K p_{+1, t}(k) \frac{o_t(k, k_{-1, t})\bfone{k_{+1, t} = k} + \beta}{p_{+1, t}(k)} = o_t(k_{+1, t}, k_{-1, t}) + K\beta.
\end{equation}
As $p_{+1, t}(k) \hat{g}_{+1, t}(k) \leq 1 + \beta$, we get
\begin{align*}
    (1 - \gamma) \sum_{t=1}^T \hat{g}_{+1, t}(j) &\leq \beta KT + \sum_{t=1}^T o_t(k_{+1, t}, k_{-1, t}) + \eta (1 + \beta) \sum_{t = 1}^T \sum_{k = 1}^K \hat{g}_{+1, t}(k) + \frac{\ln K}{\eta} \\
    &\leq \beta KT + \sum_{t=1}^T o_t(k_{+1, t}, k_{-1, t}) + \eta (1 + \beta) K \max_{k \in [K]} \sum_{t = 1}^T \hat{g}_{+1, t}(k) + \frac{\ln K}{\eta} \\
    &\leq \beta KT + \sum_{t=1}^T o_t(k_{+1, t}, k_{-1, t}) + \gamma \max_{k \in [K]} \sum_{t = 1}^T \hat{g}_{+1, t}(k) + \frac{\ln K}{\eta}
\end{align*}
The last inequality uses the fact that $\gamma \geq \eta (1 + \beta) K$ by assumption. As the inequality holds for any arbitrary $j \in [K]$, we can take a $\max$ over $j \in [K]$ on the left hand side. Simplifying this further yields:
\begin{align*}
    (1 - 2\gamma) \max_{j \in [K]} \sum_{t=1}^T \hat{g}_{+1, t}(j) \leq \beta K T + \sum_{t=1}^T o_t(k_{+1, t}, k_{-1, t}) + \frac{\ln K}{\eta}.
\end{align*}
By Azuma-Hoeffding's inequality, with probability at least $1 - \delta/2$, 
\begin{equation*}
    \sum_{t = 1}^T o_t(k_{+1, t}, k_{-1, t}) \leq \sum_{t = 1}^T P_t(k_{+1, t}, k_{-1, t}) + 2\sqrt{2T \ln(2/\delta)}.
\end{equation*}
Combining this with Lemma \ref{lemma:g_hat_upper_bounds_p_row_player}, we get with probability at least $1 - \delta$,
\begin{equation*}
    (1 - 2\gamma) \max_{j \in [K]} \left[ \sum_{t=1}^T P_t(j, k_{-1, t}) - \frac{\ln(2K/\delta)}{\beta} \right] \leq \beta KT + \sum_{t = 1}^T P_t(k_{+1, t}, k_{-1, t}) + 2\sqrt{2T \ln(2/\delta)} + \frac{\ln K}{\eta}.
\end{equation*}
Let $\gamma = 2\eta K \geq \eta (1 + \beta) K$. Then,
\begin{equation*}
    \max_{j \in [K]} \sum_{t=1}^T P_t(j, k_{-1, t}) - \sum_{t = 1}^T P_t(k_{+1, t}, k_{-1, t}) \leq \beta KT + 2\sqrt{2T \ln(2/\delta)} + \frac{\ln K}{\eta} + \frac{\ln(2K/\delta)}{\beta} + 4\eta K T.
\end{equation*}
Setting $\eta = \frac{1}{2}\sqrt{\frac{\ln K}{KT}}$ and $\beta = \sqrt{\frac{\ln K}{KT}}$ finishes the proof.

\end{proof}

==> sec/Borda.tex <==
We consider the Borda-DBwK problem where our algorithm competes against $\optb$, a solution of the LP $\eqref{lp:primal-Borda}$.
We also define the shifted borda score and the corresponding LP as follows
\begin{defn}
\label{rem:regeqv}
The \emph{shifted Borda score} of item $i \in [K]$ is $s(i) := \frac{1}{K} \sum_{j \in [K]} \P(i,j)$. 
\end{defn}
We define the benchmark LP with shifted Borda score as 
 \begin{align*}
    \max_{\pi} &\sum_{x} s(x) \pi(x) + \sum_{y} s(y) \pi(y)\\
    \text{such that } &\sum_{x} v(x) \pi(x) + \sum_{y} v(y) \pi(y) \leq \frac{B}{T} \mathbf{1}
\end{align*}
Let the solution to the above LP be $\widetilde{\pi}^*$ and let $\widetilde{\opt}$ be the associated value. Then in the following lemma we show that the optimal value with the true Borda score is some constant times the optimal value with shifted Borda score.

\begin{lemma}
    $\opt = \frac{K}{K-1}\widetilde{\opt}$
\end{lemma}

\begin{theorem}
    For $\eta = \big(\frac{\log K}{T\sqrt{T}}\big)^{2/3}\frac{1}{Z}$ and $\gamma = \sqrt{\eta K}$, the regret of B-DBwK EXP-3 is bounded by
    \begin{align*}
        R(T) \leq \tilde{\mathcal{O}}\Big(\frac{OPT}{B} (K\log K)^{2/3} T^{2/3} \Big)
    \end{align*}
\end{theorem}
\emph{Proof sketch}
Using the EXP-3 guarantee we have 
\begin{align*}
    \forall a, \; \sum_{t=1}^{\tau} \hat{\ell}_t(a) &- \sum_{t=1}^{\tau}\sum_{a} \tilde{q}_t(a)\hat{\ell}_t(a)  \\
    &\leq \frac{\log K}{\eta} + \eta \sum_{t=1}^{\tau}\sum_{i=1}^{K} \tilde{q}_t(i)\hat{\ell}_t(i)
\end{align*}
Since $\displaystyle \tilde{q}_t(i) = \frac{q_t(i) - \frac{\gamma}{K}}{1-\gamma}$,
\begin{align*}
    \forall a, \; \sum_{t=1}^{\tau} \hat{\ell}_t(a) &- \sum_{t=1}^{\tau}\sum_{a} \frac{q_t(i)}{1-\gamma}\hat{\ell}_t(a) + \frac{\frac{\gamma}{K}}{1-\gamma}\hat{\ell}_t(a) \\
    &\leq \frac{\log K}{\eta} + \eta \sum_{t=1}^{\tau}\sum_{i=1}^{K} \tilde{q}_t(i)\hat{\ell}_t(i)
\end{align*}
\begin{align*}
    \forall a, \; &\underbrace{(1-\gamma)\sum_{t=1}^{\tau} \hat{\ell}_t(a) - \sum_{t=1}^{\tau}\sum_{a} q_t(i)\hat{\ell}_t(a) + \frac{\frac{\gamma}{K}}{1-\gamma}\hat{\ell}_t(a)}_{I} \\
    &\leq \underbrace{\frac{\log K}{\eta} + \eta \sum_{t=1}^{\tau}\sum_{i=1}^{K} \tilde{q}_t(i)\hat{\ell}_t(i) - \frac{\gamma}{K}\sum_{t=1}^{\tau}\sum_{a}\hat{\ell}_t(i)}_{II}
\end{align*}

\begin{restatable}{lemm}{lemmatermone}
\label{lemma:lhs}
        Term-I can be lower bounded as follows:
        \begin{align*}
            I \geq OPT-REW - (1-\gamma)(Z+4)\sqrt{T\log T}
        \end{align*}
\end{restatable}

% \begin{lemma}
%     \label{lemma:lhs}
%         Term-I can be lower bounded as follows:
%         \begin{align*}
%             I \geq OPT-REW - (1-\gamma)(Z+4)\sqrt{T\log T}
%         \end{align*}
%     \end{lemma}
\begin{restatable}{lemm}{lemmatermtwo}
\label{lemma:rhs}
        Term-II can be upper bounded as follows:
        \begin{align*}
            II \leq \mathcal{O}\left((\log K)^{2/3}K^{2/3} T^{2/3}\frac{OPT}{B}\right)
        \end{align*}
\end{restatable}
% \begin{theorem}
%     The regret of B-DBwK-BTM is bounded by
%     $
%         R(T) \leq \tilde{\mathcal{O}}\Big(\frac{OPT}{B} \sqrt{T}\Big)
%     $
% \end{theorem}

% \begin{proof}
%     We have
%     \begin{align*}
%         s(i) &= \frac{1}{K} \sum_{j=1}^{K}P(i,j) = \frac{K-1}{K(K-1)} \sum_{j\neq i} P(i,j) + \frac{1}{2K}\\
%              &= \frac{K-1}{K} b(i) + \frac{1}{2K}.
%     \end{align*}
%     Therefore 
% \end{proof}

 \begin{algorithm}[H]
 \caption{\textbf{Vigilant D-EXP3} (for Borda Regret) }
   \label{alg:dexp3}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Item set indexed by $[K]$, learning rate $\eta > 0$, parameters $\gamma \in (0,1)$ %scale parameter $\lambda_t$
   %\STATE \quad\quad\quad\quad Confidence parameter: $\delta >0$
   \STATE {\bfseries Initialize:} Initial probability distribution $\q_1(i) = 1/K, ~\forall i \in [K]$
   \FOR {$t = 1, \ldots, T$}
   \STATE Sample $x_t, y_t \sim \q_t$ i.i.d.~(with replacement) 
   \STATE Receive preference $o_{t}(x_t,y_t) \sim \text{Ber}(\P_t(x_t,y_t))$
   \STATE Estimate scores, for all $i \in [K]$: 
   \begin{align*}
       \hat{s}_t(i) &= 
       \frac{\1(x_t = i)}{K q_t(i)}\sum_{j \in [K]}\frac{\1(y_t = j)o_t(x_t,y_t)}{q_t(j)},\\
        \hat{v}^1_t (i) &= 1 - \frac{\1(x_t = i)}{q_t(i)} (1-v_t(x_t)),\\
        \hat{v}^2_t (i) &= 1 - \frac{\1(y_t = i)}{q_t(i)} (1-v_t(y_t)).
   \end{align*}
   \STATE Compute an estimate of the Lagrangian
   \begin{align*}
       \hat{\ell}_t(i) = 2 \hat{s}_t(i) + Z \lambda_{t}^T \bigg[\frac{B}{T}\mathbbm{1} - (\hat{v}^1_t(i) + \hat{v}^2_t(i))\bigg]
   \end{align*}
   \STATE Update, for all $i \in [K]$: 
   \begin{align*}
       \hat{q}_{t+1}(i) &= \dfrac{\exp(\eta \sum_{\tau = 1}^t \hat{\ell}_\tau(i))}{\sum_{j = 1}^{K} \exp(\eta \sum_{\tau = 1}^t \hat{\ell}_\tau(j))};\\
       q_{t+1}(i) &= (1-\gamma)\hat{q}_{t+1}(i) + \frac{\gamma}{K}
   \end{align*}
    \STATE Update $\lambda_t$ using OCO on 
    $$g_{t}(\lambda) = \Big \langle \frac{B}{T} \mathbbm{1} - (u_t(x_{t}) + u_t(y_{t}))\Big \rangle$$
   \ENDFOR
   %\STATE {\bfseries Output:} 
\end{algorithmic}
\end{algorithm}
Combining Lemma~\ref{lemma:lhs} and Lemma~\ref{lemma:rhs} gives
\begin{align*}
    OPT-REW &\leq \mathcal{O}\left((\log K)^{2/3}K^{2/3} T^{2/3}\frac{OPT}{B}\right) \\
    &+ (1-\gamma)(Z+4)\sqrt{T\log T}\\
    &= \mathcal{O}\left((\log K)^{2/3}K^{2/3} T^{2/3}\frac{OPT}{B}\right)
\end{align*}


% \begin{algorithm}[H]
%  \caption{\textbf{Borda Dueling Bandits with Knapsacks-Beat the Mean, (B-DBwK-BTM)} }
%    \label{alg:borda-btm}
% \begin{algorithmic}[1]
%    \STATE {\bfseries Input:} Item set indexed by $[K]$, learning rate $\eta > 0$, parameters $\gamma \in (0,1)$ %scale parameter $\lambda_t$
%    %\STATE \quad\quad\quad\quad Confidence parameter: $\delta >0$
%    \STATE {\bfseries Initialize:} $W_1 \leftarrow \{1,2,\ldots K\}, n_k,w_k \leftarrow 0, k \in [K], q \leftarrow 1$
%    \WHILE {$|W_q|>1$ and $ t\leq T$}
%    \STATE $x_t \leftarrow \arg \min _{b\in W_q} n_b$
%    \STATE $y_t \leftarrow$ Uniformly at random from $W_q$. 
%    \STATE if $x_t$ wins, $w_x \leftarrow w_x + 1$
%    \STATE $n_x \leftarrow n_x + 1$
%    \IF{ $\min_{x \in W_q} \ell(x)^{UCB-LCB} \leq \max_{x \in W_q} \ell(y)^{LCB-UCB}$}
%     \STATE $x' \leftarrow \arg\min_{x \in W_q} \ell(x)^{UCB-LCB}$ from $W_q$
%     \STATE $W_q \leftarrow W_q \setminus \{x'\}$
%     \STATE Delete all comparisons with $x'$ from $n_k, w_k, k\in [K]$
%     \STATE $q \leftarrow q+1$
%     \ENDIF
%     \STATE $t \leftarrow t+1$
%    \ENDWHILE
%    %\STATE {\bfseries Output:} 
% \end{algorithmic}
% \end{algorithm}



==> sec/BwK_problem.tex <==
Here we describe a counter example that has sub-optimal regret for the algorithm from \citep{Badanidiyuru_2013}

\begin{algorithm}[ht]
\caption{Algorithm \pdbwk for deterministic outcomes, with parameter $\eps\in(0,1)$}
\label{alg:determ}
\begin{algorithmic}[1]
\STATE In the first $\narms$ rounds, pull each arm once.\;
\STATE  For each arm $x\in X$, let $r_x\in [0,1]$ and $C_x\in[0,1]^\nrsc$
\STATE  denote the reward and the resource consumption vector revealed in Step 2.
\STATE  $v_1 = \ones \in [0,1]^\nrsc$.
\STATE 
    \COMMENT{$v_t\in [0,1]^\nrsc$ is the round-$t$ estimate of the optimal solution $\eta^*$.}
\STATE 
    \COMMENT{We interpret $v_t(i)$ as an estimate of the (fictional) unit cost of  resource $i$, for each $i$.}
\STATE  Set $\eps = \sqrt{\ln(\nrsc)/\budg}$.
\FOR{rounds $t = \narms+1,\ldots,\stime \;\; \mbox{\it (i.e., until
resource budget exhausted)}$}
\STATE For each arm $x\in X$,
\STATE  \emph{Expected cost} for one pull of arm $x$ is estimated by $\text{EstCost}_x = C_x\cdot v_t$.
\STATE Pull arm $x=x_t\in X$ that maximizes  $r_x/\text{EstCost}_x$, the \emph{bang-per-buck} ratio.
\label{algstep:argmin-det}
\STATE Update estimated unit cost for each resource $i$:
\begin{align*}
                v_{t+1}(i) = v_t(i)\, (1+\eps)^{\ell},\;  \ell = C_x(i).
\end{align*}
\label{algstep:mwu-det}
\ENDFOR
\end{algorithmic}
\end{algorithm}

Consider two arms with deterministic rewards and consumption. Suppose the reward received by playing the first arm is $0.1$ and the reward received by playing the second arm is $1$. Further suppose there is only a single resource; the first arm consumes $0$ units and the second arm consumes $1$ unit at every arm pull. The time horizon is $T$ and the total budget available $B = \frac{T}{2}$.

Consider the following policy $\hat{\pi}$
\begin{itemize}
    \item Pull arm-2 for the first $\frac{T}{2}$ rounds and obtain total reward $\frac{T}{2}$
    \item Pull arm-1 for the next $\frac{T}{2}$ rounds and obtain total reward $\frac{0.1T}{2}$
\end{itemize}
Total reward accumulated reward, $\frac{1.1}{2}T$.

Recall that the $\texttt{LP-primal}$ is given by

\begin{align}
\begin{array}{lrcll}
	\max         & \sum_{x\in X}\, \xi_x\, r(x,\mu) & &            & \text{in $\xi_x \in \R$, for each $x\in X$} \\
	\text{s.t.}  & \sum_{x\in X} \xi_x\, c_i(x,\mu)  & \leq & B  & \text{for each resource $i$} \\
			     & \xi_x     & \geq & 0                            & \text{for each arm $x$},
\end{array}
\tag{\texttt{LP-primal}}
\end{align}

and for our setting this reduces to
\begin{align*}
    \max\;\; & 0.1 \xi_1 + \xi_2\\
    \text{s.t. } & \xi_2 \leq B
\end{align*}

Notice that for $\hat{\pi}$, we have $\xi_1 = \xi_2 = \frac{T}{2}$, is feasible and therefore the optimal reward $\opt \geq \frac{1.1}{2}T$.

The policy obtained by Algorithm~\ref{alg:determ} chooses arm-1 $T-1$ times and arm-2 once because $\text{EstCost}_{x}$ in line 11 for $x=1$ is 0. The total reward for this policy $REW = 0.1(T-1) + 1$ and the regret is 
\begin{align*}
    \reg = \opt - \rew \geq \frac{1.1}{2} T -  0.1 (T - 1) - 1 = \Omega(T)
\end{align*}

\rdcomment{This is for the deterministic algorithm. Need to construct an example that works even when we have UCB and LCB estimates of reward and consumption respectively: Probably would work with the above eg. since LCB estimate would be negative and the algorithm does $\cap$ [0,1].}

==> sec/comments.tex <==

\ascomment{1. Need to reduce focus on BwK ow there is a high chance reviewers will fail to see the novelty of our new ideas/algorithms, use BwK references as sparsely as possible.

2. Need to emphasize (in Intro+Abs) why its important to solve the budgeted DB problem

3. Contributions should precisely mention the challenges to work with Preferences in the contained case: Explain with toy examples (1 and 2 are good arms but hard to distinguish unless duel with with 3, which has high cost). Important to clearly justify why its worth writing a paper and that we are not simply copying the BwK framework and their techniques -- ``Constrained DB problem is inherently challenging since judging the utility of an item relies of comparative measurements, unlike MAB setup"

4. Have table showing what MAB results look like and our findings with their DB counterparts. Refer this table in the List of Contributions

5. Need to add few lines in the Intro and some remarks in the Alg section to justify novelty of our algorithms: It took us time to figure our where to insert the Lagrangian, what is the underlying algorithm, how to analyze it, etc

6. Use `cost' instead of consumption; `constrained/budgeted' instead of Knapsack, remove with occurrence of `BwK' (we can use something like `Frugal-DB' or {\bf {\it f}-DB}) etc. We need to use as few terminologies as possible from the BwK literature, right now its looks like we are pretty much copying their problem setup and algorithms for DB.}

\rdcomment{Separately, often in the real world the learner might also encounter a limited supply of resources and needs to satisfy one or more budget constraints along with the objective of maximizing the total reward. For example there might budget associated with the number of times a movie is shown by recommendation systems, or restrictions on the number of times an ad is shown, or constraint on the battery capacity of a mobile robot etc. Many other applications such as clinical trials, crowd sourcing, dynamic pricing often have certain constraints associated and as such one often needs to come up with algorithms for settings where the learner needs to also pay attention to consumption of resources along with trying to maximize its cumulative rewards. The Bandits with Knapsacks (BwK) formulation \citep{Badanidiyuru_2013}  provides such a framework to the learner. \citep{Badanidiyuru_2013} developed the simplest version for MAB setting, wherein at each round the agent additionally receives a vector of consumptions, each dimension corresponding to a resource. The objective of the learner is to maximize the total accumulated reward over the horizon $T$ but at the same time also ensure that the total sum of consumptions is less than a given budget for every resource. Subsequently \citep{AdCBwK} considered the constrained setting with adversarial bandits, \citep{linCBwK} extended it with linear contextual bandits and \cite{pmlr-v162-sivakumar22a} studied it in the smoothed adversarial setting.




For example clinical trials are constrained by available medical resources or optimizing for ad
placements should account for advertisers budget and user
reach.  

Although both these frameworks have received significant attention separately, the combined setting has not yet been examined. However, the intersection of both these frameworks include interesting applications such as movie recommendations, advertisement systems, search engine optimization \rdcomment{think these through}. 
In this work, we therefore develop and study the combined framework \emph{Dueling Bandits with Knapsacks} (DBwK), where the agent learns using pairwise comparisons while simultaneously satisfying budget constraints. Below we unpack our main contribution in this work.}
